Geographic distribution of the global agricultural workforce every decade for the years 2000-2100

Agricultural workers play a vital role in the global economy and food security by cultivating, transporting, and processing food for populations worldwide. Despite their importance, detailed spatial data on the global agricultural workforce have remained scarce. Here, we present a new gridded dataset that maps the global distribution of agricultural workers for every decade over the years 2000-2100, distributed at 0.083$\times$0.083 degrees resolution, roughly $\sim$10km$\times$10km at the Equator. The dataset is developed using an empirical modeling framework relying on generalized additive mixed models (GAMMs) that integrate socioeconomic variables, including gross domestic product per capita, total population, rural population size, and agricultural land use. The predictions are consistent with Shared Socio-economic Pathways and we distribute full time series data for all SSPs 1 to 5. This dataset opens new avenues for future research on labour force health, productivity and risk, and could be very useful for developing informed, forward-looking strategies that address the challenges of climate resilience in agriculture. The dataset and code for reproducing it are available for the user community [publicly available on publication at DOI: 10.5281/zenodo.14443333].

==> Tables/ag_population_changes_countries_top_changes_ssp2_2050.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{l|>{}r|>{}r|>{}r|>{}r|>{}rl}
\caption{\label{tab:top_ag_changes2050} Top 10 Countries with Largest Positive, Negative, and Smallest Changes by 2050 under SSP 2}\\
\toprule
country & region\_wb & type & baseline\_ag\_pop & future\_ag\_pop & change & percent\_change\\
\midrule
\endfirsthead
\caption[]{Top 10 Countries with Largest Positive, Negative, and Smallest Changes by 2050 under SSP 2 \textit{(continued)}}\\
\toprule
country & region\_wb & type & baseline\_ag\_pop & future\_ag\_pop & change & percent\_change\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{Niger} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{7,694,406} & \cellcolor{gray!10}{15,732,124} & \cellcolor{gray!10}{8,037,718} & \cellcolor{gray!10}{104.5\%}\\
Kuwait & MENA & Positive Change & 89,076 & 178,884 & 89,808 & 100.8\%\\
\cellcolor{gray!10}{Singapore} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{551,498} & \cellcolor{gray!10}{1,102,861} & \cellcolor{gray!10}{551,364} & \cellcolor{gray!10}{100.0\%}\\
Malawi & SSA & Positive Change & 6,258,346 & 10,977,638 & 4,719,293 & 75.4\%\\
\cellcolor{gray!10}{Uganda} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{18,043,585} & \cellcolor{gray!10}{31,206,854} & \cellcolor{gray!10}{13,163,269} & \cellcolor{gray!10}{73.0\%}\\
\addlinespace
Qatar & MENA & Positive Change & 70,212 & 118,671 & 48,459 & 69.0\%\\
\cellcolor{gray!10}{Zambia} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{4,294,649} & \cellcolor{gray!10}{6,910,274} & \cellcolor{gray!10}{2,615,625} & \cellcolor{gray!10}{60.9\%}\\
Mali & SSA & Positive Change & 7,693,885 & 11,843,108 & 4,149,222 & 53.9\%\\
\cellcolor{gray!10}{Angola} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{5,323,110} & \cellcolor{gray!10}{8,167,253} & \cellcolor{gray!10}{2,844,143} & \cellcolor{gray!10}{53.4\%}\\
United Arab Emirates & MENA & Positive Change & 171,325 & 261,489 & 90,164 & 52.6\%\\
\addlinespace
\cellcolor{gray!10}{Bahrain} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{22,612} & \cellcolor{gray!10}{34,385} & \cellcolor{gray!10}{11,773} & \cellcolor{gray!10}{52.1\%}\\
Nigeria & SSA & Positive Change & 39,676,426 & 59,139,636 & 19,463,210 & 49.1\%\\
\cellcolor{gray!10}{Afghanistan} & \cellcolor{gray!10}{SA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{7,159,828} & \cellcolor{gray!10}{10,595,188} & \cellcolor{gray!10}{3,435,360} & \cellcolor{gray!10}{48.0\%}\\
Burundi & SSA & Positive Change & 6,648,044 & 9,784,981 & 3,136,936 & 47.2\%\\
\cellcolor{gray!10}{Central African Republic} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{959,603} & \cellcolor{gray!10}{1,408,357} & \cellcolor{gray!10}{448,754} & \cellcolor{gray!10}{46.8\%}\\
\addlinespace
Madagascar & SSA & Positive Change & 10,719,275 & 15,665,500 & 4,946,225 & 46.1\%\\
\cellcolor{gray!10}{Rwanda} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{3,697,463} & \cellcolor{gray!10}{5,403,181} & \cellcolor{gray!10}{1,705,718} & \cellcolor{gray!10}{46.1\%}\\
Uruguay & LAC & Positive Change & 143,622 & 208,645 & 65,023 & 45.3\%\\
\cellcolor{gray!10}{Luxembourg} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{4,210} & \cellcolor{gray!10}{6,063} & \cellcolor{gray!10}{1,853} & \cellcolor{gray!10}{44.0\%}\\
Norway & ECA & Positive Change & 66,937 & 95,517 & 28,580 & 42.7\%\\
\addlinespace
\cellcolor{gray!10}{Belgium} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{87,693} & \cellcolor{gray!10}{89,734} & \cellcolor{gray!10}{2,041} & \cellcolor{gray!10}{2.3\%}\\
Switzerland & ECA & Smallest Change & 178,366 & 182,185 & 3,819 & 2.1\%\\
\cellcolor{gray!10}{Viet Nam} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{25,737,078} & \cellcolor{gray!10}{26,157,828} & \cellcolor{gray!10}{420,749} & \cellcolor{gray!10}{1.6\%}\\
United Kingdom of Great Britain and Northern Ireland & ECA & Smallest Change & 802,979 & 814,821 & 11,842 & 1.5\%\\
\cellcolor{gray!10}{Lao People's Democratic Republic} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{2,632,667} & \cellcolor{gray!10}{2,670,583} & \cellcolor{gray!10}{37,916} & \cellcolor{gray!10}{1.4\%}\\
\addlinespace
Panama & LAC & Smallest Change & 333,494 & 336,351 & 2,857 & 0.9\%\\
\cellcolor{gray!10}{Ecuador} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{2,087,368} & \cellcolor{gray!10}{2,103,757} & \cellcolor{gray!10}{16,389} & \cellcolor{gray!10}{0.8\%}\\
South Africa & SSA & Smallest Change & 2,079,906 & 2,094,894 & 14,988 & 0.7\%\\
\cellcolor{gray!10}{Mexico} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{5,943,941} & \cellcolor{gray!10}{5,966,441} & \cellcolor{gray!10}{22,501} & \cellcolor{gray!10}{0.4\%}\\
Papua New Guinea & EAP & Smallest Change & 596,083 & 597,089 & 1,006 & 0.2\%\\
\addlinespace
\cellcolor{gray!10}{Suriname} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{29,182} & \cellcolor{gray!10}{29,199} & \cellcolor{gray!10}{18} & \cellcolor{gray!10}{0.1\%}\\
Colombia & LAC & Smallest Change & 4,433,429 & 4,425,447 & -7,982 & -0.2\%\\
\cellcolor{gray!10}{Canada} & \cellcolor{gray!10}{NA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{550,097} & \cellcolor{gray!10}{548,239} & \cellcolor{gray!10}{-1,858} & \cellcolor{gray!10}{-0.3\%}\\
Kazakhstan & ECA & Smallest Change & 4,476,916 & 4,445,317 & -31,599 & -0.7\%\\
\cellcolor{gray!10}{Botswana} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{191,182} & \cellcolor{gray!10}{188,996} & \cellcolor{gray!10}{-2,186} & \cellcolor{gray!10}{-1.1\%}\\
\addlinespace
Nicaragua & LAC & Smallest Change & 981,196 & 966,676 & -14,520 & -1.5\%\\
\cellcolor{gray!10}{Montenegro} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{19,081} & \cellcolor{gray!10}{18,701} & \cellcolor{gray!10}{-380} & \cellcolor{gray!10}{-2.0\%}\\
Occupied Palestinian Territory & MENA & Smallest Change & 126,002 & 123,253 & -2,749 & -2.2\%\\
\cellcolor{gray!10}{Denmark} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{78,227} & \cellcolor{gray!10}{75,920} & \cellcolor{gray!10}{-2,307} & \cellcolor{gray!10}{-2.9\%}\\
Tajikistan & ECA & Smallest Change & 1,494,832 & 1,446,959 & -47,873 & -3.2\%\\
\addlinespace
\cellcolor{gray!10}{Russian Federation} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{5,906,151} & \cellcolor{gray!10}{4,719,936} & \cellcolor{gray!10}{-1,186,214} & \cellcolor{gray!10}{-20.1\%}\\
Estonia & ECA & Negative Change & 34,081 & 27,160 & -6,921 & -20.3\%\\
\cellcolor{gray!10}{Germany} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{810,959} & \cellcolor{gray!10}{638,766} & \cellcolor{gray!10}{-172,193} & \cellcolor{gray!10}{-21.2\%}\\
Poland & ECA & Negative Change & 2,493,122 & 1,928,592 & -564,530 & -22.6\%\\
\cellcolor{gray!10}{Hungary} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{271,287} & \cellcolor{gray!10}{208,594} & \cellcolor{gray!10}{-62,693} & \cellcolor{gray!10}{-23.1\%}\\
\addlinespace
Georgia & MENA & Negative Change & 733,544 & 560,369 & -173,175 & -23.6\%\\
\cellcolor{gray!10}{Armenia} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{436,381} & \cellcolor{gray!10}{330,645} & \cellcolor{gray!10}{-105,736} & \cellcolor{gray!10}{-24.2\%}\\
Croatia & ECA & Negative Change & 189,718 & 143,477 & -46,241 & -24.4\%\\
\cellcolor{gray!10}{Guyana} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{89,339} & \cellcolor{gray!10}{66,691} & \cellcolor{gray!10}{-22,648} & \cellcolor{gray!10}{-25.4\%}\\
Latvia & ECA & Negative Change & 103,091 & 75,267 & -27,824 & -27.0\%\\
\addlinespace
\cellcolor{gray!10}{French Guiana} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{6,929} & \cellcolor{gray!10}{4,892} & \cellcolor{gray!10}{-2,037} & \cellcolor{gray!10}{-29.4\%}\\
Bosnia and Herzegovina & ECA & Negative Change & 225,337 & 158,898 & -66,440 & -29.5\%\\
\cellcolor{gray!10}{Bhutan} & \cellcolor{gray!10}{SA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{230,419} & \cellcolor{gray!10}{159,916} & \cellcolor{gray!10}{-70,503} & \cellcolor{gray!10}{-30.6\%}\\
Japan & EAP & Negative Change & 3,200,007 & 2,208,958 & -991,049 & -31.0\%\\
\cellcolor{gray!10}{Democratic People's Republic of Korea} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{1,680,775} & \cellcolor{gray!10}{1,160,230} & \cellcolor{gray!10}{-520,545} & \cellcolor{gray!10}{-31.0\%}\\
\addlinespace
Serbia & ECA & Negative Change & 821,911 & 566,739 & -255,173 & -31.0\%\\
\cellcolor{gray!10}{Austria} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{222,027} & \cellcolor{gray!10}{148,559} & \cellcolor{gray!10}{-73,468} & \cellcolor{gray!10}{-33.1\%}\\
Republic of Moldova & ECA & Negative Change & 650,673 & 427,142 & -223,531 & -34.4\%\\
\cellcolor{gray!10}{Sri Lanka} & \cellcolor{gray!10}{SA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{2,980,128} & \cellcolor{gray!10}{1,664,733} & \cellcolor{gray!10}{-1,315,395} & \cellcolor{gray!10}{-44.1\%}\\
Åland Islands & ECA & Negative Change & 132 & 44 & -88 & -66.8\%\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_changes_countries_top_changes_ssp2_2100.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{l|>{}r|>{}r|>{}r|>{}r|>{}rl}
\caption{\label{tab:top_ag_changes2100} Top 20 Countries with Largest Positive, Negative, and Smallest Changes by 2100 under SSP 2}\\
\toprule
country & region\_wb & type & baseline\_ag\_pop & future\_ag\_pop & change & percent\_change\\
\midrule
\endfirsthead
\caption[]{Top 10 Countries with Largest Positive, Negative, and Smallest Changes by 2100 under SSP 2 \textit{(continued)}}\\
\toprule
country & region\_wb & type & baseline\_ag\_pop & future\_ag\_pop & change & percent\_change\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{Bahrain} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{17,857} & \cellcolor{gray!10}{99,024} & \cellcolor{gray!10}{81,167} & \cellcolor{gray!10}{454.5\%}\\
Singapore & EAP & Positive Change & 215,899 & 1,130,779 & 914,880 & 423.8\%\\
\cellcolor{gray!10}{Qatar} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{25,103} & \cellcolor{gray!10}{129,918} & \cellcolor{gray!10}{104,816} & \cellcolor{gray!10}{417.6\%}\\
Liechtenstein & ECA & Positive Change & 8 & 37 & 29 & 346.3\%\\
\cellcolor{gray!10}{Israel} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{99,345} & \cellcolor{gray!10}{331,671} & \cellcolor{gray!10}{232,326} & \cellcolor{gray!10}{233.9\%}\\
\addlinespace
Niger & SSA & Positive Change & 4,464,475 & 13,956,245 & 9,491,770 & 212.6\%\\
\cellcolor{gray!10}{Kuwait} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{87,788} & \cellcolor{gray!10}{270,087} & \cellcolor{gray!10}{182,299} & \cellcolor{gray!10}{207.7\%}\\
Uganda & SSA & Positive Change & 10,156,462 & 30,998,269 & 20,841,807 & 205.2\%\\
\cellcolor{gray!10}{Malawi} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{4,032,244} & \cellcolor{gray!10}{11,950,880} & \cellcolor{gray!10}{7,918,636} & \cellcolor{gray!10}{196.4\%}\\
United Arab Emirates & MENA & Positive Change & 91,563 & 267,614 & 176,052 & 192.3\%\\
\addlinespace
\cellcolor{gray!10}{Egypt} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{2,742,798} & \cellcolor{gray!10}{7,985,968} & \cellcolor{gray!10}{5,243,170} & \cellcolor{gray!10}{191.2\%}\\
Rwanda & SSA & Positive Change & 2,246,307 & 5,411,533 & 3,165,226 & 140.9\%\\
\cellcolor{gray!10}{Zambia} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{3,238,078} & \cellcolor{gray!10}{7,732,640} & \cellcolor{gray!10}{4,494,562} & \cellcolor{gray!10}{138.8\%}\\
Nigeria & SSA & Positive Change & 30,188,619 & 71,973,024 & 41,784,404 & 138.4\%\\
\cellcolor{gray!10}{Equatorial Guinea} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{64,656} & \cellcolor{gray!10}{141,728} & \cellcolor{gray!10}{77,072} & \cellcolor{gray!10}{119.2\%}\\
\addlinespace
Afghanistan & SA & Positive Change & 4,377,992 & 9,424,988 & 5,046,996 & 115.3\%\\
\cellcolor{gray!10}{Angola} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{4,276,641} & \cellcolor{gray!10}{9,039,463} & \cellcolor{gray!10}{4,762,822} & \cellcolor{gray!10}{111.4\%}\\
Burundi & SSA & Positive Change & 3,946,219 & 8,263,344 & 4,317,124 & 109.4\%\\
\cellcolor{gray!10}{Guatemala} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Positive Change} & \cellcolor{gray!10}{2,436,864} & \cellcolor{gray!10}{4,639,178} & \cellcolor{gray!10}{2,202,314} & \cellcolor{gray!10}{90.4\%}\\
Mali & SSA & Positive Change & 5,173,353 & 9,833,375 & 4,660,022 & 90.1\%\\
\addlinespace
\cellcolor{gray!10}{Tanzania, United Republic of} & \cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{11,177,834} & \cellcolor{gray!10}{12,348,107} & \cellcolor{gray!10}{1,170,273} & \cellcolor{gray!10}{10.5\%}\\
Occupied Palestinian Territory & MENA & Smallest Change & 102,495 & 109,568 & 7,073 & 6.9\%\\
\cellcolor{gray!10}{Canada} & \cellcolor{gray!10}{NA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{505,458} & \cellcolor{gray!10}{526,597} & \cellcolor{gray!10}{21,139} & \cellcolor{gray!10}{4.2\%}\\
Honduras & LAC & Smallest Change & 1,215,385 & 1,259,533 & 44,147 & 3.6\%\\
\cellcolor{gray!10}{Indonesia} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{31,514,785} & \cellcolor{gray!10}{32,163,118} & \cellcolor{gray!10}{648,333} & \cellcolor{gray!10}{2.1\%}\\
\addlinespace
New Zealand & EAP & Smallest Change & 105,728 & 102,802 & -2,926 & -2.8\%\\
\cellcolor{gray!10}{Australia} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{407,234} & \cellcolor{gray!10}{394,709} & \cellcolor{gray!10}{-12,526} & \cellcolor{gray!10}{-3.1\%}\\
Côte d’Ivoire & SSA & Smallest Change & 4,097,671 & 3,970,494 & -127,177 & -3.1\%\\
\cellcolor{gray!10}{Suriname} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{27,881} & \cellcolor{gray!10}{26,924} & \cellcolor{gray!10}{-957} & \cellcolor{gray!10}{-3.4\%}\\
Switzerland & ECA & Smallest Change & 190,094 & 182,827 & -7,267 & -3.8\%\\
\addlinespace
\cellcolor{gray!10}{United Kingdom of Great Britain and Northern Ireland} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{908,843} & \cellcolor{gray!10}{873,743} & \cellcolor{gray!10}{-35,100} & \cellcolor{gray!10}{-3.9\%}\\
Oman & MENA & Smallest Change & 242,812 & 230,746 & -12,066 & -5.0\%\\
\cellcolor{gray!10}{Ireland} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{135,187} & \cellcolor{gray!10}{125,889} & \cellcolor{gray!10}{-9,298} & \cellcolor{gray!10}{-6.9\%}\\
Turkmenistan & ECA & Smallest Change & 1,237,549 & 1,144,634 & -92,915 & -7.5\%\\
\cellcolor{gray!10}{Sudan} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{4,588,089} & \cellcolor{gray!10}{4,229,705} & \cellcolor{gray!10}{-358,384} & \cellcolor{gray!10}{-7.8\%}\\
\addlinespace
Sierra Leone & SSA & Smallest Change & 1,005,107 & 913,984 & -91,123 & -9.1\%\\
\cellcolor{gray!10}{Saudi Arabia} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{1,925,008} & \cellcolor{gray!10}{1,743,126} & \cellcolor{gray!10}{-181,881} & \cellcolor{gray!10}{-9.4\%}\\
Nepal & SA & Smallest Change & 7,824,241 & 7,070,990 & -753,251 & -9.6\%\\
\cellcolor{gray!10}{Republic of Korea} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Smallest Change} & \cellcolor{gray!10}{1,995,843} & \cellcolor{gray!10}{1,796,480} & \cellcolor{gray!10}{-199,364} & \cellcolor{gray!10}{-10.0\%}\\
Bolivia (Plurinational State of) & LAC & Smallest Change & 1,764,445 & 1,586,207 & -178,238 & -10.1\%\\
\addlinespace
\cellcolor{gray!10}{Austria} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{296,259} & \cellcolor{gray!10}{120,395} & \cellcolor{gray!10}{-175,864} & \cellcolor{gray!10}{-59.4\%}\\
Romania & ECA & Negative Change & 3,449,145 & 1,366,130 & -2,083,015 & -60.4\%\\
\cellcolor{gray!10}{Estonia} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{46,559} & \cellcolor{gray!10}{18,251} & \cellcolor{gray!10}{-28,307} & \cellcolor{gray!10}{-60.8\%}\\
Germany & ECA & Negative Change & 1,279,646 & 481,506 & -798,140 & -62.4\%\\
\cellcolor{gray!10}{Bulgaria} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{1,090,302} & \cellcolor{gray!10}{406,905} & \cellcolor{gray!10}{-683,397} & \cellcolor{gray!10}{-62.7\%}\\
\addlinespace
Uruguay & LAC & Negative Change & 318,859 & 118,980 & -199,879 & -62.7\%\\
\cellcolor{gray!10}{Hungary} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{399,333} & \cellcolor{gray!10}{146,453} & \cellcolor{gray!10}{-252,880} & \cellcolor{gray!10}{-63.3\%}\\
Cuba & LAC & Negative Change & 1,132,652 & 409,527 & -723,125 & -63.8\%\\
\cellcolor{gray!10}{Georgia} & \cellcolor{gray!10}{MENA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{1,085,113} & \cellcolor{gray!10}{378,128} & \cellcolor{gray!10}{-706,985} & \cellcolor{gray!10}{-65.2\%}\\
Lithuania & ECA & Negative Change & 269,189 & 87,252 & -181,936 & -67.6\%\\
\addlinespace
\cellcolor{gray!10}{Serbia} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{1,192,277} & \cellcolor{gray!10}{381,889} & \cellcolor{gray!10}{-810,389} & \cellcolor{gray!10}{-68.0\%}\\
Armenia & MENA & Negative Change & 745,017 & 235,429 & -509,587 & -68.4\%\\
\cellcolor{gray!10}{Latvia} & \cellcolor{gray!10}{ECA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{130,897} & \cellcolor{gray!10}{39,857} & \cellcolor{gray!10}{-91,040} & \cellcolor{gray!10}{-69.6\%}\\
Belarus & ECA & Negative Change & 1,429,685 & 430,641 & -999,043 & -69.9\%\\
\cellcolor{gray!10}{Guyana} & \cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{122,653} & \cellcolor{gray!10}{36,124} & \cellcolor{gray!10}{-86,528} & \cellcolor{gray!10}{-70.5\%}\\
\addlinespace
Bosnia and Herzegovina & ECA & Negative Change & 361,856 & 99,264 & -262,592 & -72.6\%\\
\cellcolor{gray!10}{Democratic People's Republic of Korea} & \cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{2,149,031} & \cellcolor{gray!10}{585,708} & \cellcolor{gray!10}{-1,563,323} & \cellcolor{gray!10}{-72.7\%}\\
Lesotho & SSA & Negative Change & 268,787 & 69,084 & -199,703 & -74.3\%\\
\cellcolor{gray!10}{Bhutan} & \cellcolor{gray!10}{SA} & \cellcolor{gray!10}{Negative Change} & \cellcolor{gray!10}{540,826} & \cellcolor{gray!10}{114,978} & \cellcolor{gray!10}{-425,848} & \cellcolor{gray!10}{-78.7\%}\\
Republic of Moldova & ECA & Negative Change & 1,047,722 & 211,363 & -836,359 & -79.8\%\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_1_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP1}\\
\toprule
region\_wb & Pop baseline & Pop SSP1 2050 & $\Delta$ Pop SSP1 2050 & Pop SSP1 2100 & $\Delta$ Pop SSP1 2100\\
\midrule
\endfirsthead
\caption[]{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP1 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP1 2050 & $\Delta$ Pop SSP1 2050 & Pop SSP1 2100 & $\Delta$ Pop SSP1 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{698.8M} & \cellcolor{gray!10}{450.4M} & \cellcolor{gray!10}{-35.5\%} & \cellcolor{gray!10}{266.4M} & \cellcolor{gray!10}{-61.9\%}\\
ECA & 48.2M & 26.0M & -46.1\% & 17.4M & -63.9\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{57.1M} & \cellcolor{gray!10}{43.6M} & \cellcolor{gray!10}{-23.7\%} & \cellcolor{gray!10}{36.2M} & \cellcolor{gray!10}{-36.6\%}\\
MENA & 37.5M & 32.6M & -13.0\% & 29.7M & -20.7\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{3.7M} & \cellcolor{gray!10}{-6.1\%} & \cellcolor{gray!10}{3.1M} & \cellcolor{gray!10}{-21.6\%}\\
SA & 351.9M & 355.2M & 0.9\% & 244.8M & -30.4\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{214.7M} & \cellcolor{gray!10}{353.6M} & \cellcolor{gray!10}{64.7\%} & \cellcolor{gray!10}{303.3M} & \cellcolor{gray!10}{41.3\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_1_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP1}\\
\toprule
region\_wb & Pop baseline & Pop SSP1 2050 & $\Delta$ Pop SSP1 2050 & Pop SSP1 2100 & $\Delta$ Pop SSP1 2100\\
\midrule
\endfirsthead
\caption[]{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP1 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP1 2050 & $\Delta$ Pop SSP1 2050 & Pop SSP1 2100 & $\Delta$ Pop SSP1 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{543.9M} & \cellcolor{gray!10}{452.3M} & \cellcolor{gray!10}{-16.8\%} & \cellcolor{gray!10}{267.8M} & \cellcolor{gray!10}{-50.8\%}\\
ECA & 45.4M & 27.8M & -38.8\% & 19.2M & -57.6\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{58.4M} & \cellcolor{gray!10}{36.4M} & \cellcolor{gray!10}{-37.6\%} & \cellcolor{gray!10}{30.0M} & \cellcolor{gray!10}{-48.6\%}\\
MENA & 36.1M & 31.6M & -12.3\% & 28.3M & -21.5\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{-0.7\%} & \cellcolor{gray!10}{4.1M} & \cellcolor{gray!10}{-11.6\%}\\
SA & 271.6M & 351.1M & 29.3\% & 241.0M & -11.3\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{193.5M} & \cellcolor{gray!10}{302.9M} & \cellcolor{gray!10}{56.5\%} & \cellcolor{gray!10}{260.0M} & \cellcolor{gray!10}{34.4\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_2_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{\label{tab:ag_predicted_2}Total Agricultural Population and Percent Change by World Bank Region}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP2 2100 & $\Delta$ Pop SSP2 2100\\
\midrule
\endfirsthead
\caption[]{Total Agricultural Population and Percent Change by World Bank Region \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP2 2100 & $\Delta$ Pop SSP2 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{543.9M} & \cellcolor{gray!10}{506.3M} & \cellcolor{gray!10}{-6.9\%} & \cellcolor{gray!10}{332.4M} & \cellcolor{gray!10}{-38.9\%}\\
ECA & 45.4M & 31.9M & -29.7\% & 25.1M & -44.8\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{58.4M} & \cellcolor{gray!10}{42.0M} & \cellcolor{gray!10}{-28.1\%} & \cellcolor{gray!10}{39.4M} & \cellcolor{gray!10}{-32.4\%}\\
MENA & 36.1M & 37.0M & 2.5\% & 35.4M & -1.7\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{4.5M} & \cellcolor{gray!10}{-2.8\%} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{-14.4\%}\\
SA & 271.6M & 430.8M & 58.6\% & 339.1M & 24.9\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{193.5M} & \cellcolor{gray!10}{382.7M} & \cellcolor{gray!10}{97.8\%} & \cellcolor{gray!10}{348.5M} & \cellcolor{gray!10}{80.1\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_3_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP3}\\
\toprule
region\_wb & Pop baseline & Pop SSP3 2050 & $\Delta$ Pop SSP3 2050 & Pop SSP3 2100 & $\Delta$ Pop SSP3 2100\\
\midrule
\endfirsthead
\caption[]{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP3 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP3 2050 & $\Delta$ Pop SSP3 2050 & Pop SSP3 2100 & $\Delta$ Pop SSP3 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{698.8M} & \cellcolor{gray!10}{572.5M} & \cellcolor{gray!10}{-18.1\%} & \cellcolor{gray!10}{484.7M} & \cellcolor{gray!10}{-30.6\%}\\
ECA & 48.2M & 34.3M & -28.9\% & 31.7M & -34.2\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{57.1M} & \cellcolor{gray!10}{62.6M} & \cellcolor{gray!10}{9.6\%} & \cellcolor{gray!10}{71.7M} & \cellcolor{gray!10}{25.5\%}\\
MENA & 37.5M & 45.2M & 20.5\% & 52.8M & 41.0\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{3.1M} & \cellcolor{gray!10}{-22.5\%} & \cellcolor{gray!10}{1.8M} & \cellcolor{gray!10}{-54.7\%}\\
SA & 351.9M & 552.9M & 57.1\% & 625.7M & 77.8\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{214.7M} & \cellcolor{gray!10}{563.2M} & \cellcolor{gray!10}{162.3\%} & \cellcolor{gray!10}{763.7M} & \cellcolor{gray!10}{255.7\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_3_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP3}\\
\toprule
region\_wb & Pop baseline & Pop SSP3 2050 & $\Delta$ Pop SSP3 2050 & Pop SSP3 2100 & $\Delta$ Pop SSP3 2100\\
\midrule
\endfirsthead
\caption[]{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP3 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP3 2050 & $\Delta$ Pop SSP3 2050 & Pop SSP3 2100 & $\Delta$ Pop SSP3 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{543.9M} & \cellcolor{gray!10}{574.5M} & \cellcolor{gray!10}{5.6\%} & \cellcolor{gray!10}{487.0M} & \cellcolor{gray!10}{-10.5\%}\\
ECA & 45.4M & 36.4M & -19.8\% & 33.4M & -26.4\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{58.4M} & \cellcolor{gray!10}{51.3M} & \cellcolor{gray!10}{-12.1\%} & \cellcolor{gray!10}{58.9M} & \cellcolor{gray!10}{0.9\%}\\
MENA & 36.1M & 44.4M & 23.1\% & 52.1M & 44.6\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{3.8M} & \cellcolor{gray!10}{-17.7\%} & \cellcolor{gray!10}{2.4M} & \cellcolor{gray!10}{-49.3\%}\\
SA & 271.6M & 546.3M & 101.1\% & 615.4M & 126.6\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{193.5M} & \cellcolor{gray!10}{478.9M} & \cellcolor{gray!10}{147.5\%} & \cellcolor{gray!10}{654.4M} & \cellcolor{gray!10}{238.2\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_4_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP4}\\
\toprule
region\_wb & Pop baseline & Pop SSP4 2050 & $\Delta$ Pop SSP4 2050 & Pop SSP4 2100 & $\Delta$ Pop SSP4 2100\\
\midrule
\endfirsthead
\caption[]{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP4 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP4 2050 & $\Delta$ Pop SSP4 2050 & Pop SSP4 2100 & $\Delta$ Pop SSP4 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{698.8M} & \cellcolor{gray!10}{437.7M} & \cellcolor{gray!10}{-37.4\%} & \cellcolor{gray!10}{232.9M} & \cellcolor{gray!10}{-66.7\%}\\
ECA & 48.2M & 25.9M & -46.3\% & 16.7M & -65.5\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{57.1M} & \cellcolor{gray!10}{44.6M} & \cellcolor{gray!10}{-21.9\%} & \cellcolor{gray!10}{37.8M} & \cellcolor{gray!10}{-33.8\%}\\
MENA & 37.5M & 36.1M & -3.6\% & 39.5M & 5.4\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{3.5M} & \cellcolor{gray!10}{-12.5\%} & \cellcolor{gray!10}{2.5M} & \cellcolor{gray!10}{-37.0\%}\\
SA & 351.9M & 373.8M & 6.2\% & 270.7M & -23.1\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{214.7M} & \cellcolor{gray!10}{436.5M} & \cellcolor{gray!10}{103.3\%} & \cellcolor{gray!10}{528.3M} & \cellcolor{gray!10}{146.1\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_4_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP4}\\
\toprule
region\_wb & Pop baseline & Pop SSP4 2050 & $\Delta$ Pop SSP4 2050 & Pop SSP4 2100 & $\Delta$ Pop SSP4 2100\\
\midrule
\endfirsthead
\caption[]{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP4 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP4 2050 & $\Delta$ Pop SSP4 2050 & Pop SSP4 2100 & $\Delta$ Pop SSP4 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{543.9M} & \cellcolor{gray!10}{439.6M} & \cellcolor{gray!10}{-19.2\%} & \cellcolor{gray!10}{234.5M} & \cellcolor{gray!10}{-56.9\%}\\
ECA & 45.4M & 27.6M & -39.1\% & 18.1M & -60.0\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{58.4M} & \cellcolor{gray!10}{37.3M} & \cellcolor{gray!10}{-36.0\%} & \cellcolor{gray!10}{31.2M} & \cellcolor{gray!10}{-46.5\%}\\
MENA & 36.1M & 35.3M & -2.1\% & 38.5M & 6.8\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{4.3M} & \cellcolor{gray!10}{-7.3\%} & \cellcolor{gray!10}{3.3M} & \cellcolor{gray!10}{-28.9\%}\\
SA & 271.6M & 369.4M & 36.0\% & 265.6M & -2.2\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{193.5M} & \cellcolor{gray!10}{372.6M} & \cellcolor{gray!10}{92.6\%} & \cellcolor{gray!10}{451.1M} & \cellcolor{gray!10}{133.2\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_5_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{\label{tab:ag_pop_ssp5_corrected}Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP5}\\
\toprule
region\_wb & Pop baseline & Pop SSP5 2050 & $\Delta$ Pop SSP5 2050 & Pop SSP5 2100 & $\Delta$ Pop SSP5 2100\\
\midrule
\endfirsthead
\caption[]{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP5 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP5 2050 & $\Delta$ Pop SSP5 2050 & Pop SSP5 2100 & $\Delta$ Pop SSP5 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{698.8M} & \cellcolor{gray!10}{450.2M} & \cellcolor{gray!10}{-35.6\%} & \cellcolor{gray!10}{268.3M} & \cellcolor{gray!10}{-61.6\%}\\
ECA & 48.2M & 26.8M & -44.5\% & 20.8M & -56.9\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{57.1M} & \cellcolor{gray!10}{43.2M} & \cellcolor{gray!10}{-24.3\%} & \cellcolor{gray!10}{38.0M} & \cellcolor{gray!10}{-33.4\%}\\
MENA & 37.5M & 32.7M & -12.8\% & 32.5M & -13.1\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{4.3M} & \cellcolor{gray!10}{7.4\%} & \cellcolor{gray!10}{4.7M} & \cellcolor{gray!10}{19.5\%}\\
SA & 351.9M & 349.9M & -0.6\% & 234.6M & -33.3\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{214.7M} & \cellcolor{gray!10}{342.0M} & \cellcolor{gray!10}{59.3\%} & \cellcolor{gray!10}{285.0M} & \cellcolor{gray!10}{32.7\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2000_2050_2100_5_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP5}\\
\toprule
region\_wb & Pop baseline & Pop SSP5 2050 & $\Delta$ Pop SSP5 2050 & Pop SSP5 2100 & $\Delta$ Pop SSP5 2100\\
\midrule
\endfirsthead
\caption[]{Uncorrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP5 \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP5 2050 & $\Delta$ Pop SSP5 2050 & Pop SSP5 2100 & $\Delta$ Pop SSP5 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{543.9M} & \cellcolor{gray!10}{452.2M} & \cellcolor{gray!10}{-16.9\%} & \cellcolor{gray!10}{270.6M} & \cellcolor{gray!10}{-50.3\%}\\
ECA & 45.4M & 28.8M & -36.5\% & 24.5M & -46.0\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{58.4M} & \cellcolor{gray!10}{36.2M} & \cellcolor{gray!10}{-38.0\%} & \cellcolor{gray!10}{31.9M} & \cellcolor{gray!10}{-45.4\%}\\
MENA & 36.1M & 31.7M & -12.1\% & 31.2M & -13.6\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{5.3M} & \cellcolor{gray!10}{13.6\%} & \cellcolor{gray!10}{6.8M} & \cellcolor{gray!10}{45.4\%}\\
SA & 271.6M & 345.4M & 27.2\% & 231.1M & -14.9\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{193.5M} & \cellcolor{gray!10}{293.1M} & \cellcolor{gray!10}{51.5\%} & \cellcolor{gray!10}{245.2M} & \cellcolor{gray!10}{26.7\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2010_2050_2100_2_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Total Agricultural Population and Percent Change by World Bank Region}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP2 2100 & $\Delta$ Pop SSP2 2100\\
\midrule
\endfirsthead
\caption[]{Total Agricultural Population and Percent Change by World Bank Region \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & \$\textbackslash{}Delta\$ Pop SSP2 2050 & Pop SSP2 2100 & \$\textbackslash{}Delta\$ Pop SSP2 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{143.2M} & \cellcolor{gray!10}{135.1M} & \cellcolor{gray!10}{-5.6\%} & \cellcolor{gray!10}{113.4M} & \cellcolor{gray!10}{-20.8\%}\\
ECA & 37.9M & 31.8M & -16.0\% & 25.0M & -34.0\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{41.5M} & \cellcolor{gray!10}{42.9M} & \cellcolor{gray!10}{3.3\%} & \cellcolor{gray!10}{40.3M} & \cellcolor{gray!10}{-2.9\%}\\
MENA & 32.5M & 37.0M & 14.0\% & 35.1M & 8.3\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.7M} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{-2.8\%} & \cellcolor{gray!10}{4.1M} & \cellcolor{gray!10}{-12.5\%}\\
\addlinespace
SA & 379.4M & 430.7M & 13.5\% & 354.3M & -6.6\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{222.1M} & \cellcolor{gray!10}{378.7M} & \cellcolor{gray!10}{70.5\%} & \cellcolor{gray!10}{345.5M} & \cellcolor{gray!10}{55.5\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2010_2050_2_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llll}
\caption{Total Agricultural Population and Percent Change by World Bank Region}\\
\toprule
WB Region & Baseline & SSP2 2050 & $\Delta$ Population\\
\midrule
\endfirsthead
\caption[]{Total Agricultural Population and Percent Change by World Bank Region under business as usual development. Baseline year is 2010. \textit{(continued)}}\\
\toprule
WB Region & Baseline & SSP2 2050 & $\Delta$ Population\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{861.5M} & \cellcolor{gray!10}{758.9M} & \cellcolor{gray!10}{-11.9\%}\\
ECA & 39.4M & 31.6M & -19.9\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{51.5M} & \cellcolor{gray!10}{58.5M} & \cellcolor{gray!10}{13.6\%}\\
MENA & 41.3M & 46.1M & 11.6\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{5.6M} & \cellcolor{gray!10}{5.2M} & \cellcolor{gray!10}{-7.0\%}\\
SA & 371.0M & 422.4M & 13.9\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{283.1M} & \cellcolor{gray!10}{579.9M} & \cellcolor{gray!10}{104.8\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2010_2050_2_predicted_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llll}
\caption{Total Agricultural Population and Percent Change by World Bank Region}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050\\
\midrule
\endfirsthead
\caption[]{Total Agricultural Population and Percent Change by World Bank Region \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{593.1M} & \cellcolor{gray!10}{519.0M} & \cellcolor{gray!10}{-12.5\%}\\
ECA & 36.6M & 30.9M & -15.5\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{41.3M} & \cellcolor{gray!10}{43.8M} & \cellcolor{gray!10}{5.9\%}\\
MENA & 33.6M & 38.0M & 13.2\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.8M} & \cellcolor{gray!10}{4.6M} & \cellcolor{gray!10}{-3.9\%}\\
\addlinespace
SA & 377.7M & 457.7M & 21.2\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{222.0M} & \cellcolor{gray!10}{403.2M} & \cellcolor{gray!10}{81.6\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_2020_2050_2100_2_corrected_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP2}\\
\toprule
WB Region & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP2 2100 & $\Delta$ Pop SSP2 2100\\
\midrule
\endfirsthead
\caption[]{Corrected Predictions of Total Agricultural Population and Percent Change by World Bank Region under scenario SSP2 \textit{(continued)}}\\
\toprule
WB Region & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP2 2100 & $\Delta$ Pop SSP2 2100\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{422.5M} & \cellcolor{gray!10}{377.0M} & \cellcolor{gray!10}{-10.8\%} & \cellcolor{gray!10}{250.1M} & \cellcolor{gray!10}{-40.8\%}\\
ECA & 34.4M & 30.1M & -12.4\% & 23.2M & -32.6\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{51.2M} & \cellcolor{gray!10}{51.7M} & \cellcolor{gray!10}{0.9\%} & \cellcolor{gray!10}{48.6M} & \cellcolor{gray!10}{-5.1\%}\\
MENA & 37.8M & 39.1M & 3.5\% & 38.4M & 1.6\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{3.9M} & \cellcolor{gray!10}{3.7M} & \cellcolor{gray!10}{-6.3\%} & \cellcolor{gray!10}{3.1M} & \cellcolor{gray!10}{-21.8\%}\\
\addlinespace
SA & 402.4M & 438.7M & 9.0\% & 349.0M & -13.3\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{314.8M} & \cellcolor{gray!10}{451.5M} & \cellcolor{gray!10}{43.4\%} & \cellcolor{gray!10}{411.4M} & \cellcolor{gray!10}{30.7\%}\\*
\end{longtable}
\endgroup{}


==> Tables/ag_population_table_wb.tex <==
\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{llllll}
\caption{Total Agricultural Population and Percent Change by World Bank Region}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & $\Delta$ Pop SSP2 2050 & Pop SSP5 2050 & $\Delta$ Pop SSP5 2050\\
\midrule
\endfirsthead
\caption[]{Total Agricultural Population and Percent Change by World Bank Region \textit{(continued)}}\\
\toprule
region\_wb & Pop baseline & Pop SSP2 2050 & \$\textbackslash{}Delta\$ Pop SSP2 2050 & Pop SSP5 2050 & \$\textbackslash{}Delta\$ Pop SSP5 2050\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!10}{EAP} & \cellcolor{gray!10}{718.8M} & \cellcolor{gray!10}{452.4M} & \cellcolor{gray!10}{-37.1\%} & \cellcolor{gray!10}{448.5M} & \cellcolor{gray!10}{-37.6\%}\\
ECA & 51.2M & 25.4M & -50.4\% & 23.6M & -54.0\%\\
\cellcolor{gray!10}{LAC} & \cellcolor{gray!10}{67.6M} & \cellcolor{gray!10}{45.8M} & \cellcolor{gray!10}{-32.3\%} & \cellcolor{gray!10}{40.7M} & \cellcolor{gray!10}{-39.8\%}\\
MENA & 58.6M & 48.0M & -18.1\% & 43.0M & -26.6\%\\
\cellcolor{gray!10}{NA} & \cellcolor{gray!10}{4.7M} & \cellcolor{gray!10}{3.4M} & \cellcolor{gray!10}{-27.1\%} & \cellcolor{gray!10}{4.0M} & \cellcolor{gray!10}{-16.1\%}\\
SA & 381.3M & 485.2M & 27.3\% & 442.5M & 16.1\%\\
\cellcolor{gray!10}{SSA} & \cellcolor{gray!10}{260.1M} & \cellcolor{gray!10}{348.3M} & \cellcolor{gray!10}{33.9\%} & \cellcolor{gray!10}{313.5M} & \cellcolor{gray!10}{20.5\%}\\*
\end{longtable}
\label{tab:region_stats}
\endgroup{}


==> Tables/input_data_features.tex <==
\begin{table}[H]
    \centering
    \caption{Summary of Data Inputs for Analysis}
    \begin{tabular}{|p{4cm}|p{6cm}|p{4cm}|}
        \hline
        \textbf{Input Feature} & \textbf{Description} & \textbf{Data Source} \\ \hline
        \textbf{Cropland and Pasture Lands} & Proportion of land areas used as cropland (land for cultivating food) and pasture lands (land for grazing animals) at 5 arc-minute resolution for the year 2000. & \cite{ramankutty_farming_2008} \\ \hline
        \textbf{Rural and Urban Population Size} & Rural and urban population size data downscaled to 1-km resolution, originally published at 7.5 arc-minute resolution. & \cite{gao2017downscaling}, \cite{Jones_2016} \\ \hline
        \textbf{Median GDP} & Median of the GDP distribution (to proxy economic opportunity) estimated at 30 arc-second resolution for the year 2020. & \cite{wang_global_2022} \\ \hline
    \end{tabular}
    \label{tab:data_inputs}
\end{table}

==> Tables/ml_projections.tex <==
\begin{table}[H]
\centering
\caption{Projected Changes in Agricultural Workforce by 2050 Across Regions.}
\begin{tabular}{lrrr}
\toprule
Region & Current (M) & Change by 2050 (M) & Percent Change (\%) \\
\midrule
EAP   & 422.0 & -1.3 & -0.31 \\
ECA   & 51.9  & 2.3  & 4.43 \\
LAC   & 45.6  & -0.0864  & -0.19 \\
MENA  & 22.8  & 0.4289  & 1.88 \\
NA    & 3.7   & 0.0159  & 0.43 \\
SA    & 306.3 & -0.4197 & -0.14 \\
SSA   & 237.3 & 6.0   & 2.53 \\
\bottomrule
\end{tabular}
\label{tab:ml_projections}
\end{table}


==> Tables/model_comparison_table.tex <==
\begin{table}[H]
\centering
\caption{Model Comparison Table}
\centering
\begin{tabular}[t]{lrrr}
\toprule
Model & AIC & GCV.UBRE & Deviance.Explained\\
\midrule
linear model & 2.303667e+12 & 1.151834e+12 & 0.5462783\\
smooth terms & 8.232254e+11 & 4.116128e+11 & 0.6904333\\
smooth terms + RE, 50th & 7.375310e+11 & 3.687656e+11 & 0.8940029\\
smooth terms + RE, 80th & 1.532757e+05 & 7.701070e+04 & 0.6748897\\
interactions, 50th & 7.381692e+11 & 3.690847e+11 & 0.8856497\\
\addlinespace
interactions, 80th & 7.356305e+11 & 3.678153e+11 & 0.8854276\\
\bottomrule
\end{tabular}
\label{tab:model_comparison}
\end{table}

